Scalable Video Object Segmentation with Identification Mechanism

This paper delves into the challenges of achieving scalable and effective multi-object modeling for semi-supervised Video Object Segmentation (VOS). Previous VOS methods decode features with a single positive object, limiting the learning of multi-object representation as they must match and segment each target separately under multi-object scenarios. Additionally, earlier techniques catered to specific application objectives and lacked the flexibility to fulfill different speed-accuracy requirements. To address these problems, we present two innovative approaches, Associating Objects with Transformers (AOT) and Associating Objects with Scalable Transformers (AOST). In pursuing effective multi-object modeling, AOT introduces the IDentification (ID) mechanism to allocate each object a unique identity. This approach enables the network to model the associations among all objects simultaneously, thus facilitating the tracking and segmentation of objects in a single network pass. To address the challenge of inflexible deployment, AOST further integrates scalable long short-term transformers that incorporate scalable supervision and layer-wise ID-based attention. This enables online architecture scalability in VOS for the first time and overcomes ID embeddings' representation limitations. Given the absence of a benchmark for VOS involving densely multi-object annotations, we propose a challenging Video Object Segmentation in the Wild (VOSW) benchmark to validate our approaches. We evaluated various AOT and AOST variants using extensive experiments across VOSW and five commonly used VOS benchmarks, including YouTube-VOS 2018 & 2019 Val, DAVIS-2017 Val & Test, and DAVIS-2016. Our approaches surpass the state-of-the-art competitors and display exceptional efficiency and scalability consistently across all six benchmarks. Project page: https://github.com/yoxu515/aot-benchmark.

==> Figures/40objects.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{Sources/40objects.pdf}

    \caption{Panoptic propagation. Our method performs well when propagating the panoptic annotations of two complex scenarios (with 44/43 objects) from VIPSeg~\cite{Miao_2022_CVPR}.}
    \label{fig:40objects}

\end{figure}

==> Figures/aost.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{.26\textwidth}
			\centering
			\includegraphics[width=\textwidth]{Sources/before_aost.pdf}
			\caption{No scalability}\label{fig:before_aost}
\end{subfigure}
\vspace{2mm}
\begin{subfigure}[b]{.26\textwidth}
			\centering
			\includegraphics[width=\textwidth]{Sources/after_aost.pdf}

			\caption{Scalable VOS (ours)}\label{fig:after_aost}
\end{subfigure}
\vspace{2mm}
\begin{subfigure}[b]{.4\textwidth}
			\centering
			\includegraphics[width=\textwidth]{Sources/aost.pdf}
			\caption{AOST framework}\label{fig:overview_aost}
\end{subfigure}

\caption{(a) Previous VOS methods are not flexible for different deployment requirements. (b) Our Associating Objects with Scalable Transformers (AOST) approach supports dynamic run-time adjustment for speed-accuracy trade-offs. (c) An illustration of AOST. Here, the Scalable LSTT (S-LSTT) has 3 layers of LSTT Block V2, which utilizes improved attention functions (Fig.~\ref{fig:block_v2}) with layer-wise identification and gating weights. During training, all the sub-networks' ($L'=1/2/3$) predictions ($Y'_{1/2/3}$) are supervised by our scalable supervision.}\label{fig:aost}
\end{figure*}

==> Figures/attention.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{Sources/visual_attention.pdf}

    \caption{Visualization of long-term and short-term attention maps during the inference of DAVIS 2017~\cite{davis2017}. There are three similar people, marked in different colors, in the video. We use AOT-B, where only the first frame is considered into the long-term memory, to verify the effect of long-term attention. We propagate the colored multi-object masks in long-term or short-term memory to the current frame regarding the corresponding attention map for visualization. The brighter the color, the stronger the attention. $l=1$, $2$, and $3$ denote the 3 LSTT layers of AOT-B in order.}
    \label{fig:attention}

\end{figure}

==> Figures/davis2017.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{Sources/davis.pdf}

    \caption{Qualitative results on DAVIS 2017~\cite{davis2017}.}
    \label{fig:davis2017}

\end{figure}

==> Figures/id_bank.tex <==
% \begin{figure}[t!]
% \begin{center}

% \begin{subfigure}[t]{.24\linewidth}
% 			\centering
% 			\includegraphics[width=0.9\linewidth]{Sources/id_bank_10_nobg.png}
% 			\caption{$M=10$}\label{fig:id_bank_10}
% \end{subfigure}
% \begin{subfigure}[t]{.24\linewidth}
% 			\centering
% 			\includegraphics[width=0.9\linewidth]{Sources/id_bank_15_nobg.png}
% 			\caption{$M=15$}\label{fig:id_bank_15}
% \end{subfigure}
% \begin{subfigure}[t]{.24\linewidth}
% 			\centering
% 			\includegraphics[width=0.9\linewidth]{Sources/id_bank_20_nobg.png}
% 			\caption{$M=20$}\label{fig:id_bank_20}
% \end{subfigure}
% \begin{subfigure}[t]{.24\linewidth}
% 			\centering
% 			\includegraphics[width=0.9\linewidth]{Sources/id_bank_30_nobg.png}
% 			\caption{$M=30$}\label{fig:id_bank_30}
% \end{subfigure}

% \end{center}

% \caption{Visualization of the cosine similarity between every two of $M$ identification vectors in the identity bank. We use a $M\times M$ symmetric matrix to visualize all the similarities, and diagonal values equal 1. The darker the color, the higher the similarity. When $M=10$, the similarities are stable and balanced. As $M$ increases, the matrix becomes less smooth, making the similarities unstable.}\label{fig:id_bank}
% \end{figure}

==> Figures/merge.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{Sources/merge.pdf}

    \caption{A demonstration of Dynamic Merge Augmentation. For each sampled training sequence $s$, the augmentation will sample another sequence $s'$ from different scenario and merge the objects of $s'$ into $s$.}
    \label{fig:merge}

\end{figure}

==> Figures/occlusion.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.93\linewidth]{Sources/occlusion.pdf}

%     \caption{Visualization of long-term and short-term attention maps of AOT-B on DAVIS 2017~\cite{davis2017}. The video has three similar people, marked in different colors, and the red person is occluded in frame $t-1$. For visualization, we propagate the colored multi-object masks in long-term or short-term memory to the current frame regarding the corresponding attention maps. The brighter the color, the stronger the attention. 
%     % Here, the red person is occluded in Frame $t-1$, and thus the short-term attention fails to match the person. However, the long-term attention generates an accurate attention map with a clean background in the last layer, $l=3$, resulting in a correct prediction.
%     }
%     \label{fig:occlusion}

% \end{figure}

==> Figures/overview.tex <==
\begin{figure*}[t!]
\begin{center}

\begin{subfigure}[b]{.354\textwidth}
			\centering
			\includegraphics[width=0.95\textwidth]{Sources/overview.pdf}
			\caption{Overview}\label{fig:overview}
\end{subfigure}
\hspace{2mm}
\begin{subfigure}[b]{.263\textwidth}
			\centering
			\includegraphics[width=\textwidth]{Sources/id.pdf}

			\caption{Identity assignment}\label{fig:id}
\end{subfigure}
\hspace{2mm}
\begin{subfigure}[b]{.263\textwidth}
			\centering
			\includegraphics[width=\textwidth]{Sources/lstt.pdf}
			\caption{$l$-th LSTT block}\label{fig:lstt}
\end{subfigure}

\end{center}

\caption{(a) The overview of Associating Objects with Transformers (AOT). The multi-object masks are embedded by using our identification mechanism. Moreover, a $L$-layer Long Short-Term Transformer is responsible for matching multiple objects uniformly and hierarchically. (b) An illustration of the IDentity assignment (ID) designed for transferring a $N$-object mask into an identification embedding. (c) The structure of an LSTT block. LN: layer normalization~\cite{ln}.}\label{fig:aot_overview}
\end{figure*}

==> Figures/youtubevos.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{Sources/ytb.pdf}

    \caption{Qualitative results on the validation 2019 split of YouTube-VOS~\cite{youtubevos}. Our AOT-L performs well under many challenging multi-object cases, including similar objects, occlusion, and fast motion, etc.}
    \label{fig:youtubevos}

\end{figure}

==> Tables/davis2016.tex <==
\begin{table}
% \begin{wraptable}[13]{r}{0.45\textwidth}
\begin{center}
% \vspace{-6.5mm}
\caption{The quantitative evaluation on the single-object DAVIS 2016~\cite{davis2016}.}\label{tab:davis2016}

\setlength{\tabcolsep}{7pt}
\begin{tabular}{l c c c c}
\toprule[1.5pt]
 Methods  & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & FPS \\
\midrule[1pt]
%PReM~\cite{premvos}    & 86.8  & 84.9  & 88.6  & 0.03 \\
% STM~\cite{spacetime}   &  89.3 & 88.7  & 89.9  & 6.3 \\
CFBI\pub{ECCV20}~\cite{cfbi}   & 89.4  & 88.3 & 90.5  & 6.3 \\
CFBI+\pub{TPAMI22}~\cite{cfbip}   & 89.9  & 88.7 & 91.1  & 5.9 \\
RPCM\pub{AAAI22}~\cite{rpcm}  &  90.6  & 87.1  & 94.0 & 5.8 \\
HMMN\pub{ICCV21}~\cite{hmmn}   &  90.8 & {89.6}  & {92.0}  & 10.0 \\
STCN\pub{NeurIPS21}~\cite{cheng2021stcn}   &  91.6 & {90.8}  & {92.5}  & 27.2$^\star$ \\
\hline
\hline
AOT-T  &  86.8  & 86.1 & 87.4 & \textbf{51.4} \\
AOST ($L'=1$)  & 90.5 & 89.3 & 91.7 & {38.6} \\
R50-AOST ($L'=1$)  & 90.3 & 89.6 & 90.9 & {37.4} \\
SwinB-AOST ($L'=1$)  & 92.1 & 90.4 & 93.7 & {17.9} \\
\hline
AOT-S  &  89.4  & 88.6 & 90.2 & 40.0 \\
AOST ($L'=2$)  & 90.9 & 89.5 & 92.2 & {24.8} \\
R50-AOST ($L'=2$)  & 92.0 & 90.5 & 93.4 & {24.3} \\
SwinB-AOST ($L'=2$)  & 92.2 & 90.5 & 93.8 & {14.4} \\
\hline
AOT-B  &  89.9  & 88.7 & 91.1 & 29.6 \\
AOT-L  &  {90.4}  & {89.6} & {91.1} & 18.7 \\
AOST ($L'=3$)  & 91.6 & 90.1 & 93.0 & {18.2} \\
R50-AOT-L  &  {91.1}  & {90.1} & {92.1} & 18.0 \\
R50-AOST ($L'=3$)  & 92.1 & 90.6 & 93.6 & {17.5} \\
SwinB-AOT-L  &  {92.0}  & {90.7} & {93.3} & 12.1 \\
SwinB-AOST ($L'=3$)  & \textbf{92.4} & 90.5 & \textbf{94.2} & {12.0} \\
\hline
R50-AOST-L  & {91.4} & {90.3} & {92.5} & 17.5 \\
SwinB-AOST-L  & \textbf{92.4} & \textbf{90.6} & {94.1} & 12.0 \\
\hline
% R50-AOST-L (MS)  & {84.9} & {82.3} & {87.5} & 18.0 \\
SwinB-AOST ($L'=3$, MS)  & \textbf{93.0} & {91.5} & \textbf{94.5} & 1.3 \\
SwinB-AOST-L (MS)  & \textbf{93.0} & \textbf{91.6} & {94.4} & 1.3 \\

\bottomrule[1.5pt]

\end{tabular}
\end{center}
% \end{wraptable}
\end{table}

==> Tables/new_param_compare.tex <==
\begin{table*}[h!]
\begin{center}
\caption{Efficiency comparisons on YouTube-VOS 2019 (Y-19)~\cite{youtubevos} and DAVIS-2017 (D-17)~\cite{davis2017}. Our approaches yield superior results at a faster speed with significantly fewer parameters utilized. Besides, our AOST facilitates on-the-fly architecture adjustment for optimum speed-accuracy trade-offs.}\label{tab:param}

\renewcommand\arraystretch{1.4}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{|cc|cc|cc|
>{\columncolor[HTML]{F9FFF9}}c 
>{\columncolor[HTML]{F9FBFF}}c 
>{\columncolor[HTML]{F9FBFF}}c 
>{\columncolor[HTML]{F9FBFF}}c |
>{\columncolor[HTML]{F9FFF9}}c 
>{\columncolor[HTML]{F9FBFF}}c 
>{\columncolor[HTML]{F9FBFF}}c 
>{\columncolor[HTML]{F9FBFF}}c |
>{\columncolor[HTML]{F9FFF9}}c 
>{\columncolor[HTML]{F9FBFF}}c 
>{\columncolor[HTML]{F9FBFF}}c 
>{\columncolor[HTML]{F9FBFF}}c |}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FAFAFA}}                                                                                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}}                                               & \cellcolor[HTML]{FAFAFA}                                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}}                                                        & \cellcolor[HTML]{FAFAFA}                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}}                                               & \multicolumn{3}{c|}{\cellcolor[HTML]{FAFAFA}AOST}                                                                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}}                                               & \multicolumn{3}{c|}{\cellcolor[HTML]{FAFAFA}AOST}                                                                                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}}                                               & \multicolumn{3}{c|}{\cellcolor[HTML]{FAFAFA}AOST}                                                                                                         \\ \cline{8-10} \cline{12-14} \cline{16-18} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}Method}}                                                                                                & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{CFBI\\\cite{cfbi}}}} & \multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{CFBI+\\\cite{cfbip}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{STCN\\\cite{cheng2021stcn}}}} & \multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{PCVOS\\\cite{pcvos_cvpr22}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{AOT-L\\\cite{aot}}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}${n_l'}$=3} & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}${n_l'}$=2} & \cellcolor[HTML]{FAFAFA}${n_l'}$=1 & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{AOT-L\\\cite{aot}}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}${n_l'}$=3} & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}${n_l'}$=2} & \cellcolor[HTML]{FAFAFA}${n_l'}$=1 & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{AOT-L\\\cite{aot}}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}${n_l'}$=3}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FAFAFA}${n_l'}$=2} & \cellcolor[HTML]{FAFAFA}${n_l'}$=1 \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FAFAFA}Backbone}                                                                                                                & \multicolumn{2}{c|}{\cellcolor[HTML]{FAFAFA}ResNet-101~\cite{resnet}}                                                                                                  & \multicolumn{2}{c|}{\cellcolor[HTML]{FAFAFA}ResNet-50~\cite{resnet}}                                                                                                                   & \multicolumn{4}{c|}{\cellcolor[HTML]{FAFAFA}MobileNet-V2~\cite{sandler2018mobilenetv2}}                                                                                                                                                              & \multicolumn{4}{c|}{\cellcolor[HTML]{FAFAFA}ResNet-50~\cite{resnet}}                                                                                                                                                                                 & \multicolumn{4}{c|}{\cellcolor[HTML]{FAFAFA}Swin-Base~\cite{swin}}                                                                                                                                                                                      \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FAFAFA}}                                                                   & \cellcolor[HTML]{FAFAFA}$\mathcal{J}\&\mathcal{F}$ & \multicolumn{1}{c|}{81.0}                                                                   & 82.6                                                                     & \multicolumn{1}{c|}{82.7}                                                                            & 84.6                                                                            & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}83.7}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}84.4}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}83.6}       & \cellcolor[HTML]{F9FBFF}80.5       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}84.1}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}\underline{84.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}84.3}       & 81.5                               & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}84.5}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}\textbf{85.0}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}84.8}       & 82.7                               \\ \cline{2-18} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{Y-19 Val\\\cite{youtubevos}}}}           & \cellcolor[HTML]{FAFAFA}FPS                        & \multicolumn{1}{c|}{3.4}                                                                    & 4.0                                                                      & \multicolumn{1}{c|}{8.4}                                                                             & 10.5                                                                            & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}16.0}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}15.9}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}21.9}       & \textbf{34.4}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}14.9}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}14.9}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}20.2}       & \underline{30.9}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}9.3}                                            & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}9.3}           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}11.0}       & \textbf{13.5}                      \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FAFAFA}}                                                                   & \cellcolor[HTML]{FAFAFA}$\mathcal{J}\&\mathcal{F}$ & \multicolumn{1}{c|}{75.0}                                                                   & 78.0                                                                     & \multicolumn{1}{c|}{76.1}                                                                            & -                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}78.3}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}79.5}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}78.1}       & 72.7                               & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}79.6}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}\underline{79.9}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}78.1}       & 71.2                               & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}81.2}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}\textbf{82.7}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}81.7}       & 78.6                               \\ \cline{2-18} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{FAFAFA}\makecell{D-17 Test\\\cite{davis2016}}}} & \cellcolor[HTML]{FAFAFA}FPS                        & \multicolumn{1}{c|}{5.3}                                                                    & 3.4                                                                      & \multicolumn{1}{c|}{19.5}                                                                            & -                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}18.7}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}18.2}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}24.8}       & \textbf{38.6}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}18.0}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}17.5}       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}24.3}       & \underline{37.4}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}12.1}                                           & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}12.0}          & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBFF}14.4}       & \textbf{17.9}                      \\ \hline
\multicolumn{2}{|c|}{Param (M)}                                                                                                                                       & \multicolumn{1}{c|}{66.1}                                                                   & 74.3                                                                     & \multicolumn{1}{c|}{54.5}                                                                            & 62.2                                                                            & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}\textbf{8.3}}                                   & \multicolumn{3}{c|}{\cellcolor[HTML]{F9FBFF}\textbf{8.8}}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}\underline{14.9}}                                     & \multicolumn{3}{c|}{\cellcolor[HTML]{F9FBFF}\underline{15.4}}                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FFF9}65.4}                                           & \multicolumn{3}{c|}{\cellcolor[HTML]{F9FBFF}65.9}                                                                                                         \\ \hline
\end{tabular}
\end{center}
\end{table*}


==> Tables/youtubevos.tex <==
\begin{table*}[t!]
	\centering
	\caption{The quantitative evaluation on multi-object benchmarks, YouTube-VOS~\cite{youtubevos} and DAVIS 2017~\cite{davis2017}. AOST-L shares the structure of AOST ($L'=3$) but does not use scalable supervision and has no scalability.
	AF: using \textit{All-Frames} (30FPS) videos instead of default (6FPS) videos in inference. P: parameter number (M).
	$^{\star}$: recorded on our device.
	-Y: without using YouTube-VOS for training. 
	$^{*}$: using 600p instead of 480p videos in inference. $^{\ddag}$: timing extrapolated from single-object speed assuming linear scaling in the number of objects. 
	 (MS): using test-time multi-scale and flipping augmentations.
	}\label{tab:comparisons}
	
\begin{subtable}[t]{.54\textwidth}
\centering
\caption{YouTube-VOS}\label{tab:youtubevos}
\setlength{\tabcolsep}{4pt}
% \small

\begin{tabular}{lcccccccc}
	
\toprule[1.5pt]
            & &  &  \multicolumn{2}{c}{Seen}  &    \multicolumn{2}{c}{Unseen} & &   \\
\midrule[1pt]
 Methods & AF & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & FPS & Param \\
\midrule[1pt]
\multicolumn{9}{c}{\textit{Validation 2018 Split}} \\
\midrule[1pt]
STM\pub{ICCV19}~\cite{spacetime}  & \checkmark &  79.4  &  79.7  &  84.2  &  72.8  &  80.9 & - & 34.0 \\

KMN\pub{ECCV20}~\cite{KMN}  & \checkmark &  81.4  &  81.4  &  85.6  &  75.3  &  83.3 & - & - \\
CFBI\pub{ECCV20}~\cite{cfbi} & &  81.4  &  81.1  & 85.8  & 75.3  & 83.4 & 3.4 & 66.1 \\
LWL\pub{ECCV20}~\cite{LWLVOS} & \checkmark & 81.5  &  80.4  &  84.9  &  76.4  &  84.4 & - & 36.7 \\
SST\pub{CVPR21}~\cite{sstvos} & - & 81.7  &  81.2  &  -  &  76.0  &  - & - & - \\
HMMN\pub{ICCV21}~\cite{hmmn} & \checkmark & 82.6  &  82.1  &  87.0  &  76.8  &  84.6 & - & 42.8 \\
CFBI+\pub{TPAMI22}~\cite{cfbip} & &  82.8  &  81.8  & 86.6  & 77.1  & 85.6 & 4.0 &  74.3 \\
STCN\pub{NeurIPS21}~\cite{cheng2021stcn} & \checkmark &  83.0  &  81.9  & 86.5  & 77.9  & 85.7 & 8.4$^\star$ & 54.5 \\
RPCM\pub{AAAI22}~\cite{rpcm} & &  84.0  &  83.1  & 87.7  & 78.5  & 86.7 & - & 66.4 \\
\hline
\hline
AOT-T & & 80.2  &  80.1  & 84.5  & 74.0  & 82.2 & \textbf{41.0} & \textbf{5.7} \\
AOST ($L'=1$) & & 80.6  &  80.0  & 84.8  & 74.7  & 83.1 & 34.4 & 5.8 \\
R50-AOST ($L'=1$) & & 81.6  &  81.4  & 86.1  & 75.5  & 83.5 & 30.9 & 12.5 \\
SwinB-AOST ($L'=1$) & & 82.6  &  82.7  & 87.6  & 76.2  & 84.0 & 13.5 & 62.9 \\
\hline
AOT-S & & 82.6  &  82.0  & 86.7  & 76.6  & 85.0 & {27.1} & 7.0 \\
AOST ($L'=2$) & & 83.7  &  82.8  & 87.7  & 77.7  & 86.4 & 21.9 & 7.3 \\
R50-AOST ($L'=2$) & & 84.5  &  83.5  & 88.5  & 78.8  & 87.2 & 20.2 & 13.9 \\
SwinB-AOST ($L'=2$) & & 84.7  &  84.2  & 89.2  & 78.5  & 86.9 & 11.0 & 64.4 \\
\hline
AOT-B & & 83.5  &  {82.6}  & 87.5  & {77.7}  & 86.0 & 20.5 & 8.3 \\
AOT-L & & {83.8}  &  {82.9}  & {87.9}  & {77.7}  & {86.5} & 16.0 & 8.3 \\
AOST ($L'=3$) & & 84.4  &  83.5  & 88.5  & 78.4  & 87.0 & 15.9 & 8.8 \\
R50-AOT-L & & {84.1}  &  {83.7}  & {88.5}  & {78.1}  & {86.1} & 14.9 & 14.9 \\
R50-AOST ($L'=3$) & & 85.0  &  83.8  & 88.8  & 79.3  & 87.9 & 14.9 & 15.4 \\
SwinB-AOT-L & & {84.5}  &  {84.3}  & {89.3}  & {77.9}  & {86.4} & 9.3 & 65.4 \\
SwinB-AOST ($L'=3$) & & 84.9  &  84.5  & 89.6  & 78.6  & 87.0 & 9.3 & 65.9 \\
\hline
AOST-L & & {84.5}  &  {83.5}  & {88.6}  & {78.7}  & {87.1} & 15.9 & 8.5 \\
R50-AOST-L & & {84.8}  &  {84.1}  & {88.9}  & {78.8}  & {87.3} & 14.9 & 15.1 \\
SwinB-AOST-L & & \textbf{85.1}  &  \textbf{84.5}  & \textbf{89.4}  & \textbf{79.0}  & \textbf{87.5} & 9.3 & 65.6 \\
\hline
R50-AOST-L & \checkmark & {85.4}  &  \textbf{85.1}  & \textbf{90.2}  & {78.9}  & {87.3} & 6.3 & 15.1 \\
SwinB-AOST-L & \checkmark & \textbf{85.8}  &  \textbf{85.1}  & {90.1}  & \textbf{79.6}  & \textbf{88.2} & 5.1 & 65.6 \\
SwinB-AOST-L (MS) & \checkmark & \textbf{86.5}  &  \textbf{85.6}  & \textbf{90.7}  & \textbf{80.7}  & \textbf{88.9} & 0.7 & 65.6 \\
\midrule[1pt]
\multicolumn{9}{c}{\textit{Validation 2019 Split}} \\
\midrule[1pt]
CFBI\pub{ECCV20}~\cite{cfbi}  & &  81.0  &  {80.6}  & {85.1}  & {75.2}  & {83.0} & 3.4 &  66.1 \\
SST\pub{CVPR21}~\cite{sstvos} & - & 81.8  &  80.9  &  -  &  76.6  &  - & - & - \\
HMMN\pub{ICCV21}~\cite{hmmn} & \checkmark & 82.5  &  81.7  &  86.1  &  77.3  &  85.0 & - & 42.8 \\
CFBI+\pub{TPAMI22}~\cite{cfbip} & &  82.6  &  81.7  & 86.2  & 77.1  & 85.2 & 4.0 & 74.3 \\
STCN\pub{NeurIPS21}~\cite{cheng2021stcn} & \checkmark &  82.7  &  81.1  & 85.4  & 78.2  & 85.9 & 8.4$^\star$ & 54.5 \\
RPCM\pub{AAAI22}~\cite{rpcm} & &  83.9  &  82.6  & 86.9  & 79.1  & 87.1 & - & 66.4 \\
\hline
\hline
AOT-T & &  79.7  &  79.6  & 83.8  & 73.7  & 81.8 & \textbf{41.0} & \textbf{5.7} \\
AOST ($L'=1$) & & 80.5  &  79.4  & 83.8  & 75.3  & 83.6 & 34.4 & 5.8 \\
R50-AOST ($L'=1$) & & 81.5  &  81.0  & 85.6  & 75.8  & 83.8 & 30.9 & 12.5 \\
SwinB-AOST ($L'=1$) & & 82.7  &  82.5  & 87.3  & 76.5  & 84.3 & {13.5} & 62.9 \\
\hline
AOT-S & &  82.2 &  81.3  & 85.9  & 76.6  & 84.9 & {27.1} & 7.0 \\
AOST ($L'=2$) & & 83.6  &  82.3  & 87.1  & 78.3  & 86.8 & 21.9 & 7.3 \\
R50-AOST ($L'=2$) & & 84.3  &  83.3  & 88.0  & 78.9  & 87.1 & {20.2} & 13.9 \\
SwinB-AOST ($L'=2$) & & 84.8  &  84.1  & 88.9  & 79.0  & 87.3 & {11.0} & 64.4 \\
\hline
AOT-B & &  83.3 &  {82.4}  & {87.1}  & 77.8  & 86.0 & 20.5 & 8.3 \\
AOT-L & &  {83.7} &  {82.8}  & {87.5}  & {78.0}  & {86.7} & 16.0 & 8.3 \\
AOST ($L'=3$) & & 84.4  & 83.3  & 88.0  & 79.0  & 87.4 & {15.9} & 8.8 \\
R50-AOT-L & & {84.1}  &  {83.5}  & {88.1}  & {78.4}  & {86.3} & 14.9 & 14.9 \\
R50-AOST ($L'=3$) & & 84.9 &  83.8  & 88.7  & 79.3  & 87.7 & {14.9} & 15.4 \\
SwinB-AOT-L & & {84.5}  &  {84.0}  & {88.8}  & {78.4}  & {86.7} & 9.3 & 65.4 \\
SwinB-AOST ($L'=3$) & & 85.0  &  84.5  & 89.3  & 79.0  & 87.3 & {9.3} & 65.9 \\
\hline
AOST-L & & {84.2}  &  {82.9}  & {87.8}  & {79.0}  & {87.2} & 15.9 & 8.5 \\
R50-AOST-L & & {85.0}  &  {84.0}  & {88.7}  & {79.5}  & {87.9} & 14.9 & 15.1 \\
SwinB-AOST-L & & \textbf{85.2}  &  \textbf{84.2}  & \textbf{88.9}  & \textbf{79.8}  & \textbf{88.0} & 9.3 & 65.6 \\
\hline
R50-AOST-L & \checkmark & {85.3}  &  {84.7}  & {89.6}  & {79.2}  & {87.6} & 6.3 & 15.1 \\
SwinB-AOST-L & \checkmark & \textbf{86.0}  &  \textbf{85.0}  & \textbf{89.8}  & \textbf{80.3}  & \textbf{88.8} & 5.1 & 65.6 \\
SwinB-AOST-L (MS) & \checkmark & \textbf{86.5}  &  \textbf{85.5}  & \textbf{90.3}  & \textbf{81.0}  & \textbf{89.1} & 0.7 & 65.6 \\

\bottomrule[1.5pt]
\end{tabular}

\end{subtable}
\begin{subtable}[t]{.45\textwidth}










\caption{DAVIS 2017}\label{tab:davis}
\begin{center}
% \small
\vspace{-1.8mm}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c c c c}
\toprule[1.5pt]
 Methods  & $\mathcal{J}\&\mathcal{F}$ & $\mathcal{J}$ & $\mathcal{F}$ & FPS \\
\midrule[1pt]
\multicolumn{5}{c}{\textit{Validation 2017 Split}} \\
\midrule[1pt]
%LWL\pub{ECCV20}~\cite{LWLVOS}  &  81.6  & 79.1  & 84.1 & 2.5$^\ddag$ \\
FEEL\pub{CVPR19}~\cite{feelvos}  &  71.5  &  69.1  & 74.0 & 2.0 \\
STM\pub{ICCV19}~\cite{spacetime}   &  81.8  & 79.2  & 84.3 & 3.1$^\ddag$ \\
LWL\pub{ECCV20}~\cite{LWLVOS} &  81.6  & 79.1  & 84.1 & 2.5$^\ddag$ \\
CFBI\pub{ECCV20}~\cite{cfbi}  &  81.9  & 79.3  & 84.5 & 5.9 \\
SST\pub{CVPR21}~\cite{sstvos} &  82.5  & 79.9  & 85.1 & - \\
KMN\pub{ECCV20}~\cite{KMN} (-Y)  &  76.0  & 74.2  & 77.8 & 4.2$^\ddag$ \\
KMN\pub{ECCV20}~\cite{KMN}  &  82.8  & 80.0  & 85.6 & 4.2$^\ddag$ \\
CFBI+\pub{TPAMI22}~\cite{cfbip}  &  82.9  & 80.1  & 85.7 & 5.6 \\
RPCM\pub{AAAI22}~\cite{rpcm}  &  83.7  & 81.3  & 86.0 & - \\
HMMN\pub{ICCV21}~\cite{hmmn}  &  84.7  & 81.9  & 87.5 & 5.0$^\ddag$ \\
STCN\pub{NeurIPS21}~\cite{cheng2021stcn}  &  85.4  & 82.2  & 88.6 & 24.7$^\star$ \\
\hline
\hline
AOT-T  & 79.9 & 77.4 & 82.3 & \textbf{51.4} \\
AOST ($L'=1$)  & 81.4 & 78.7 & 84.1 & {38.6} \\
R50-AOST ($L'=1$)  & 83.7 & 81.2 & 86.1 & {37.4} \\
SwinB-AOST ($L'=1$)  & 83.0 & 80.0 & 86.0 & {17.9} \\
\hline
AOT-S (-Y)  &  79.2  & 76.4 & 82.0 & 40.0 \\
AOT-S  & 81.3 & 78.7 & 83.9 & {40.0} \\
AOST ($L'=2$)  & 83.3 & 80.4 & 86.2 & {24.8} \\
R50-AOST ($L'=2$)  & 85.3 & 82.5 & 88.0 & {24.3} \\
SwinB-AOST ($L'=2$)  & 85.3 & 82.2 & 88.3 & {14.4} \\
\hline
AOT-B  & 82.5 & 79.7 & 85.2 & 29.6 \\
AOT-L  & {83.8} & {81.1} & {86.4} & 18.7 \\
AOST ($L'=3$)  & 84.2 & 81.2 & 87.2 & {18.2} \\
R50-AOT-L  & {84.9} & {82.3} & {87.5} & 18.0 \\
R50-AOST ($L'=3$)  & 85.6 & 82.6 & 88.5 & {17.5} \\
SwinB-AOT-L  & {85.4} & {82.4} & {88.4} & 12.1 \\
SwinB-AOST ($L'=3$)  & 85.5 & 82.4 & 88.6 & {12.0}\\
\hline
R50-AOST-L  & {85.3} & {82.3} & {88.2} & 17.5 \\
SwinB-AOST-L  & \textbf{86.3} & \textbf{83.1} & \textbf{89.4} & 12.0 \\
\hline
% R50-AOST-L (MS)  & {86.3} & {83.6} & {88.9} & 1.5 \\
SwinB-AOST ($L'=3$, MS)  & {86.7} & {83.8} & {89.5} & 1.3 \\
SwinB-AOST-L (MS)  & \textbf{87.0} & \textbf{84.2} & \textbf{89.8} & 1.3 \\


\midrule[1pt]
\multicolumn{5}{c}{\textit{Testing 2017 Split}} \\
\midrule[1pt]
STM\pub{ICCV19}$^{*}$~\cite{spacetime} &  72.2  & 69.3  & 75.2 & - \\
CFBI\pub{ECCV20}~\cite{cfbi}  &  75.0  & 71.4  & 78.7 & 5.3 \\
STCN\pub{NeurIPS21}~\cite{cheng2021stcn}  &  76.1  & 72.7  & 79.6 & 19.5$^\star$ \\
CFBI\pub{ECCV20}$^{*}$~\cite{cfbi}  &  76.6  & 73.0  & 80.1 & 2.9 \\
KMN\pub{ECCV20}$^{*}$~\cite{KMN}   &  77.2  & 74.1  & 80.3 & - \\
CFBI+\pub{TPAMI22}$^{*}$~\cite{cfbip}  &  78.0  & 74.4  & 81.6 & 3.4 \\
HMMN\pub{ICCV21}~\cite{hmmn}  &  78.6  & 74.7  & 82.5 & 3.4$^\ddag$ \\
RPCM\pub{AAAI22}~\cite{rpcm}  &  79.2  & 85.8  & 86.2 & - \\

\hline
\hline
AOT-T  & 72.0 & 68.3 & 75.7 & \textbf{51.4} \\
AOST ($L'=1$)  & 72.7 & 69.7 & 75.8 & {38.6} \\
R50-AOST ($L'=1$)  & 71.2 & 68.0 & 74.4 & {37.4} \\
SwinB-AOST ($L'=1$)  & 78.6 & 74.9 & 82.2 & {17.9} \\
\hline
AOT-S  &  73.9  & 70.3 & 77.5 & 40.0 \\
AOST ($L'=2$)  & 78.1 & 74.3 & 82.0 & {24.8} \\
R50-AOST ($L'=2$)  & 78.1 & 74.5 & 81.7 & {24.3} \\
SwinB-AOST ($L'=2$)  & 81.7 & 78.0 & 85.4 & {14.4} \\
\hline
AOT-B   &  75.5  & 71.6 & 79.3 & 29.6 \\
AOT-L   &  78.3  & 74.3 & 82.3 & 18.7 \\
AOST ($L'=3$)  & 79.5 & 75.6 & 83.3 & {18.2} \\
R50-AOT-L  & {79.6} & {75.9} & {83.3} & 18.0 \\
R50-AOST ($L'=3$)  & 79.9 & 76.2 & 83.6 & {17.5} \\
SwinB-AOT-L  & {81.2} & {77.3} & {85.1} & 12.1 \\
SwinB-AOST ($L'=3$)  & \textbf{82.7} & \textbf{78.8} & \textbf{86.6} & {12.0} \\
\hline
R50-AOST-L  & {80.3} & {76.7} & {83.9} & 17.5 \\
SwinB-AOST-L  & {81.9} & {78.2} & {85.6} & 12.0 \\
\hline
% R50-AOST-L (MS)  & {83.0} & {79.5} & {86.5} & 1.5 \\
SwinB-AOST ($L'=3$, MS)  & \textbf{84.7} & {80.9} & \textbf{88.5} & 1.3 \\
SwinB-AOST-L (MS)  & {84.5} & \textbf{81.0} & {87.9} & 1.3 \\
\bottomrule[1.5pt]

\end{tabular}
\end{center}

\end{subtable}

\end{table*}






